Towards Automated Polyp Segmentation Using Weakly- and Semi-Supervised Learning and Deformable Transformers

Polyp segmentation is a crucial step towards computer-aided diagnosis of colorectal cancer. However, most of the polyp segmentation methods require pixel-wise annotated datasets. Annotated datasets are tedious and time-consuming to produce, especially for physicians who must dedicate their time to their patients. We tackle this issue by proposing a novel framework that can be trained using only weakly annotated images along with exploiting unlabeled images. To this end, we propose three ideas to address this problem, more specifically our contributions are: 1) a novel sparse foreground loss that suppresses false positives and improves weakly-supervised training, 2) a batch-wise weighted consistency loss utilizing predicted segmentation maps from identical networks trained using different initialization during semi-supervised training, 3) a deformable transformer encoder neck for feature enhancement by fusing information across levels and flexible spatial locations. Extensive experimental results demonstrate the merits of our ideas on five challenging datasets outperforming some state-of-the-art fully supervised models. Also, our framework can be utilized to fine-tune models trained on natural image segmentation datasets drastically improving their performance for polyp segmentation and impressively demonstrating superior performance to fully supervised fine-tuning.

==> tex/abbrev.tex <==
% \newcommand{\jing}[1]{\textcolor{cyan}{#1}}
% \newcommand{\mich}[1]{\textcolor{olive}{#1}}
% \newcommand{\guan}[1]{\textcolor{blue}{#1}}

==> tex/introduction.tex <==
\section{Introduction}
\label{sec:intro}

Polyp segmentation is a crucial step Salient object detection (SOD) \jing{pls see comments} aims at detecting the most discriminative features \jing{for example?} in an image. Many different SOD detectors have been proposed over the years. The overwhelming majority of these works addresses the supervised SOD task, that is assuming access to pixel-wise annotated images \cite{fpn_guangyu}. However, pixel-wise annotations require significant human labour and are extremely time-consuming which makes SOD hard to be used in tasks where there is not enough labeled data and the cost of labeling is very high \jing{such as medical imaging segmentation}. This is one of the main issues for automating SOD tasks where labeled data does not exist, therefore training models with weakly annotated data for SOD is of great interest.

Computer-aided diagnosis is an area that can benefit significantly from SOD models since many tasks can be automated and save time for patients as well as physicians \jing{pls see comments}. SOD can be used for numerous medical applications such as segmentation of different types of tumours \cite{automatic_seg_review}, skin lesions \cite{skin_lesion}, cell nuclei \cite{nuclei_segmentation}, lung nodule \cite{lung_nodule} etc. However, labeling accurate pixel-wise annotations %and designing network structures 
is tedious and time-consuming for physicians. The lack of pixel-wise annotated medical data along with the lack \jing{need evidence to support this statement.} of SOD methods \jing{designed particularly for them} %that can be trained without the use of pixel-wise annotations
\jing{lead} to the bottleneck of computer aided medical diagnosis.





%---------------------------------------FIGURE---------------------------------------------------#
\begin{figure}
\minipage{0.1\textwidth}
  \centering
  \includegraphics[width=\linewidth]{latex/images/603.png}
    (a)
\endminipage\hfill
\minipage{0.1\textwidth}
  \centering
  \includegraphics[width=\linewidth]{latex/images/GT.png}
    (b) 
\endminipage\hfill
\minipage{0.1\textwidth}
  \centering
  \includegraphics[width=\linewidth]{latex/images/603——exam.png}
    (c)
\endminipage\hfill
\minipage{0.1\textwidth}
  \centering
  \includegraphics[width=\linewidth]{latex/images/sparse.png}
    (d)
\endminipage\hfill

\minipage{0.1\textwidth}
  \centering
  \includegraphics[width=\linewidth]{latex/images/rgb.png}
    (e)
\endminipage\hfill
\minipage{0.1\textwidth}
  \centering
  \includegraphics[width=\linewidth]{latex/images/GT180.png}
    (f)
\endminipage\hfill
\minipage{0.1\textwidth}
  \centering
  \includegraphics[width=\linewidth]{latex/images/fully.png}
    (g)
\endminipage\hfill
\minipage{0.1\textwidth}
  \centering
  \includegraphics[width=\linewidth]{latex/images/detr+semi.png}
    (h)
\endminipage\hfill

\caption{Visualization of Sparse annotations. (a) RGB image of training data. (b) Original ground truth (c) Our sparse annotations. (d) RGB image of testing data. (e) Prediction of fully supervised training manner. (f) Prediction of our methods. }
\label{fig:loss comparison}
\end{figure}
%---------------------------------------FIGURE---------------------------------------------------#



%In order to bridge this gap in literature and work towards achieving efficient computer aided diagnosis we ask the following questions:
% \begin{enumerate}
%     \item how could we leverage pre-trained SOD models from different domains and adapt them for medical image segmentation?
%     \item How could we use sparse-labeled and completely unlabeled medical image datasets to achieve good segmentation performance?
% \end{enumerate}
In order to bridge this gap in literature and work towards achieving efficient computer aided diagnosis we investigated: a) how to transfer knowledge from pre-trained SOD models that were trained in different domains in a fully supervised manner for medical segmentation tasks, b) how to use sparse-labeled and completely unlabeled data to achieve respectable segmentation performance as a way to address the problem of lack of pixel-wise annotated medical data. To tackle the aforementioned issues, \jing{we first create a novel dataset by sparsely relabeling half of an existing polyp training dataset with random sketches.} we \jing{further} propose a novel pipeline based on transfer learning \jing{and beyond} by adapting pre-trained models to task specific medical segmentation using only sparsely-annotated data along with unlabeled data. \jing{Moved forward} To this end we created a novel dataset by sparsely relabel half of an existing polyp training dataset with random sketches. 

Our dataset \jing{Change to: The dataset we used} contains 1,450 medical images in total and has been adapted from \jing{what does this mean} the widely used dataset from previous works \cite{fan2020pranet,ronneberger2015unet,wu2021collaborative}. However the difference is that our dataset contains only sparsely labeled data in contrast to other versions of the dataset. %As a way to visualize our dataset,
Figure \ref{fig:label percent} \jing{Why Figure 1 is not used before Figure 2?}visualises the percentage of labeled pixels on the entire training data. Apparently, including foreground and background pixels, only around 1.9\% of pixels are labeled in total and others are left as unknown pixels, which indicates that our new dataset is extremely sparse and provides the potential for achieving medical segmentation in an efficient way. Therefore, physicians will benefit significantly from an effective pipeline that can detect polyps without much labour cost.

We propose a novel pipeline leveraging our sparsely-labeled dataset to train a weakly-semi-supervised \jing{Keep the term same as title} polyp detection model. Also, we propose a novel algorithmic component as an extension of DETR \cite{DETR}  
% \jing{Frist vision transformer for WSSS https://openaccess.thecvf.com/content/CVPR2022/papers/Ru_Learning_Affinity_From_Attention_End-to-End_Weakly-Supervised_Semantic_Segmentation_With_Transformers_CVPR_2022_paper}
that provides a significant performance boost in the weakly-semi-supervised polyp detection. The robustness and generality of our proposed DETR module is further shown as it provides performance boost in the standard supervised polyp segmentation \jing{Why mention supervised? Why detection?}.

%----------------------------------------------------------------------------
\begin{figure}
\minipage{0.15\textwidth}
  \centering
  \includegraphics[width=\linewidth]{latex/images/GT180.png}
    (a)
\endminipage\hfill
\minipage{0.15\textwidth}
  \centering
  \includegraphics[width=\linewidth]{latex/images/baseline180.png}
    (b) 
\endminipage\hfill
\minipage{0.15\textwidth}
  \centering
  \includegraphics[width=\linewidth]{latex/images/baselin180_2.png}
    (c)
\endminipage\hfill

\caption{Difference between predictions of the same backbone. (a) Ground truth. (b) Prediction in the first training (c) Prediction in the second training. \alert{what is the first and second training} }
\label{fig: weak issues}
\end{figure}
%--------------------------------------------------------------------------#

It is demonstrated in \cite{zhang2020weakly,yu2021structure} that sparse annotations contain only a small part of the whole object region so directly training models by partial cross-entropy loss \cite{tang2018normalized} could cause large false positives. In order to achieve high-quality saliency maps, previous works use edge information through the use of an auxiliary edge detection network to further supervise the model and align image edges with the predicted segmentation map boundaries \cite{zhang2020weakly}. However, in our work, we take a simpler approach without extra information by proposing a novel foreground loss function that suppresses false positives and refines the rough predicted segmentation maps for weakly-supervised training.

In addition, because of the weakly-supervised training, inconsistent segmentation maps can be generated by two same models with the same training strategy. More specifically, as illustrated in Figure \ref{fig: weak issues}, due to the sparse annotations and weakly-supervised manner, both Figure \ref{fig: weak issues}(b) and Figure \ref{fig: weak issues}(c) can be treated as satisfactorily predicted segmentation maps. Therefore we propose a novel weighted consistency loss to exploit two predicted segmentation maps and refine the final predicted maps during semi-supervised training. 



%\alert{Needs to be changed somehow}Due to the lack of sparse-labeled medical datasets, we relabel half of an existing polyp training dataset with random sketches. This polyp training dataset contains 1,450 medical images in total and is widely used in previous work \cite{fan2020pranet,ronneberger2015unet,wu2021collaborative}. Figure \ref{fig:label percent} exhibits the percentage of labeled pixels on the entire training data. Apparently, including foreground and background pixels, only around 1.9\% of pixels are labeled in total and others are left as unknown pixels, which indicates that our new dataset is extremely sparse and provides the potential for achieving medical segmentation in an efficient way. Therefore, physicians benefit significantly from an effective pipeline that can detect polyps without much labour cost. In order to tackle this issue we propose a novel pipeline that can be trained using only a small number of annotated data.% polyp segmentation etc. where SOD will benefit patients by automating the


Our main contributions are \jing{Highly similar to the above 2 paragraphs}:
\begin{itemize}
    \item We release a weakly annotated dataset W-Polyp of 1,450 images by relabeling 750 images with sparse annotations, and the rest are completely unlabelled. \jing{This sentence can be deleted:}This dataset can that can be used to investigate transfer learning for salient object detection algorithms.
    \item \jing{exchange with the last contribution, or move to the begining of this paragraph} We are the first, to the best of our knowledge, to address the problem of transfer learning for salient object detection \jing{in a specific field. Make our claim safe}.
    We present a complete pipeline that takes an already pre-trained salient object detector from a different domain and fine-tunes for polyp segmentation through half of the training data which contains sparse annotations.
    
    % We investigate the problem in weakly-supervised training and design a simple weighted consistency loss to obtain weak knowledge priors for semi-supervised learning.
    \item We propose a weighted foreground loss to mitigate the issue of false positives in predicted segmentation maps for weakly-supervised learning. In addition, we investigate the inconsistent problem caused by weakly-supervised training and design a simple weighted consistency loss to refine the predicted maps in semi-supervised training.
    \item We propose several components that provide significant performance boost to our pipeline, namely fine-tuning an already pre-trained network using weakly annotated labels, leveraging unlabelled data in a semi-supervised manner, and proposing the \textbf{DefSegNet} \jing{Give a name to the detr network?} to use multi-scale deformable self-attention along with a novel progressive compensation sequence as a method for feature enhancement \alert{Jing Complete}.
\end{itemize}





\begin{figure}[H]
%\minipage{0.8\textwidth}
\centering
\includegraphics[width=0.8\linewidth]{latex/images/percentages masks.pdf}

\caption{ Percentage of labeled pixels in the new dataset. Only half of the training set is labeled with sparse annotations.}
\label{fig:label percent}
\end{figure}





